FLEXtime: Filterbank learning to explain time series

State-of-the-art methods for explaining predictions from time series involve learning an instance-wise saliency mask for each time step; however, many types of time series are difficult to interpret in the time domain, due to the inherently complex nature of the data. Instead, we propose to view time series explainability as saliency maps over interpretable parts, leaning on established signal processing methodology on signal decomposition. Specifically, we propose a new method called FLEXtime that uses a bank of bandpass filters to split the time series into frequency bands. Then, we learn the combination of these bands that optimally explains the model's prediction. Our extensive evaluation shows that, on average, FLEXtime outperforms state-of-the-art explainability methods across a range of datasets. FLEXtime fills an important gap in the current time series explainability methodology and is a valuable tool for a wide range of time series such as EEG and audio. Code is available at https://github.com/theabrusch/FLEXtime.

==> oldintro.tex <==
Explainability of black-box models is paramount for safe decision-making in critical domains such as health care \cite{amann2020a,beger2024a} and finance \cite{weber2024a}. Although recent years have seen an abundance of explainability methods developed for images \cite{achtibat2023a,fong2019a,Kolek2022,rise,relax}, time series have been overlooked to a higher degree \cite{di2023a}. A possible reason for this might be the inherently complex nature of time series \cite{rojat2021a}, making it difficult for humans to disentangle salient information. 

Explainability methods in general can be divided into local and global explanations. In this paper, we focus on local methods. Local explainability methods provide explanations for single samples of data. Local methods often produce explanations as saliency maps over input features \cite{lrp,guided-backprop,integratedgradients} leaving the interpretation of the explanation to the user. Moreover, many methods are based on smoothness and sparsity constraints, assuming localized and sparse information in the domain being explained \cite{dynamask,fong2019a,Kolek2022}. This behavior may not be suitable for explaining time series, where salient information may often be found in latent feature domains such as the frequency domain \cite{schroeder2023a}. 
Consider the case where a class is characterized by the presence of two specific frequency components. This behavior would be neither localized nor sparse if represented in the time domain. The concept is illustrated in Figure \ref{fig:time_freq} with explanations in time and frequency domain plotted as green heatmaps.
\begin{figure}
    \centering
    \includegraphics{figs/time_freq_example.pdf}
    \caption{Explainability methods that provide explanations in the time domain fail to sparsely explain time series data if the salient information is localized in the frequency domain.}
    \label{fig:time_freq}
\end{figure}

State-of-the-art methods for explaining time series often rely on learnable masks to create attribution maps in the time domain \cite{dynamask,extrmask,timexplusplus,contralsp,timex}. The masks are learned through gradient descent using an objective function that encourages the model's output on the masked version of the input data to be as close as possible to the original output while masking out as much of the input as possible. However, while these methods yield high performance on time series with salient information localized in the time domain, none of them are able to describe salient features in the frequency domain. 

In this work, we investigate learning the explanation in the frequency domain. Specifically, we first extend existing methods to the frequency domain by learning masks that zero out frequency components and present FreqDynamask. 
However, directly manipulating the frequency response by zeroing out components goes against established signal processing literature \cite{oppenheim2010a}, as it may lead to artifacts in the masked signal.

To avoid the known drawbacks of zeroing out frequency components, we therefore propose a new explainability method entitled Filterbank Learning for EXplaining time series (FLEXtime). FLEXtime defines a filterbank that divides the time series into a number of frequency bands. We then learn the explanation as the optimal combination of frequency bands. This approach has a number of advantages: It reduces the dimensionality of the problem to make for easier optimization by leveraging the fact that frequency information is often localized in bands. It obeys established principles from signal processing by properly filtering the signals. Finally, it allows for flexibility of the user to define filterbanks that are often used within specific domains, potentially allowing for a higher degree of interpretability of the learned explanations. 
Our contributions are as follows:

% Two recent works have developed new explainability methods for providing explanations for time series in the frequency domain, namely Vielhaben et al. \cite{vilrp} and Brüsch et al. \cite{freqrise}. However, the first approach relies on layer-wise relevance propagation, a gradient-based method with provable failure cases \cite{bilodeau2024a}. Additionally, gradient-based methods have been outperformed in multiple cases when providing explanations in the time domain \cite{dynamask, timexplusplus}. The second approach samples masks for directly removing frequency content with two immediate caveats; zeroing out frequency components may lead to artifacts, and computational inefficiency due to a high number of needed samples. 

% Most work on explainability for time series have used learnable masks to create attribution maps in the time domain achieving state-of-the-art performance \cite{dynamask, extrmask, timex, contralsp, timexplusplus}. The masks are learned through stochastic gradient descent using an objective function that encourages the model's output on the masked version of the input data to be as close as possible to the original output while masking out as much of the input as possible. To our knowledge, learnable masks have not been applied in the frequency domain as of yet, despite the known importance of frequency representations when analyzing time series. 

% We first show that the approach can be directly extended to learn masks in the frequency domain. However, directly manipulating the frequency response by zeroing out components goes against established signal processing literature \cite{oppenheim2010a}. For this reason, we progress to suggest Filterbank Learning for EXplaining time series (FLEXtime). FLEXtime defines a filterbank that divides the time series into a number of frequency bands. We then learn the explanation as the optimal combination of frequency bands. This approach has a number of advantages: It reduces the dimensionality of the problem to make for easier optimization. It obeys established principles from signal processing by properly filtering the signals. Finally, it allows for flexibility of the user to define filterbanks that are often used within specific domains, potentially allowing for a higher degree of interpretability of the learned explanations. 
% Our contributions are as follows:
\begin{itemize}
    \item[$\bullet$] We leverage the time-frequency duality to provide meaningful explanations in the frequency domain for time series data.
    \item[$\bullet$] We present FreqDynamask, an extension of the established baseline Dynamask \cite{dynamask} that computes saliency maps over frequency components instead of time steps. 
    \item[$\bullet$] We propose FLEXtime, which instead of masking directly in the frequency domain divides the signals into frequency bands using a filterbank. 
    \item[$\bullet$] We evaluate FLEXtime across a number of synthetic and real datasets with a range of descriptive metrics. FLEXtime beats all baselines by achieving the best average rank on faithfulness, robustness, and smoothness and the second best rank on complexity. 
    %Overall, FLEXtime gives a stable good performance, achieving the best average rank across datasets on faithfulness and robustness and the second best rank on complexity.
\end{itemize}

